The Epistemic Planning Domain Definition Language: Official Guideline

Epistemic planning extends (multi-agent) automated planning by making agents' knowledge and beliefs first-class aspects of the planning formalism. One of the most well-known frameworks for epistemic planning is Dynamic Epistemic Logic (DEL), which offers an rich and natural semantics for modelling problems in this setting. The high expressive power provided by DEL make DEL-based epistemic planning a challenging problem to tackle both theoretically, and in practical implementations. As a result, existing epistemic planners often target different DEL fragments, and typically rely on ad hoc languages to represent benchmarks, and sometimes no language at all. This fragmentation hampers comparison, reuse, and systematic benchmark development. We address these issues by introducing the Epistemic Planning Domain Definition Language (EPDDL). EPDDL provides a unique PDDL-like representation that captures the entire DEL semantics, enabling uniform specification of epistemic planning tasks. Our main contributions are: 1. A formal development of abstract event models, a novel representation for epistemic actions used to define the semantics of our language; 2. A formal specification of EPDDL's syntax and semantics grounded in DEL with abstract event models. Through examples of representative benchmarks, we illustrate how EPDDL facilitates interoperability, reproducible evaluation, and future advances in epistemic planning.

==> img/examples/multi-agent-bw/multi-agent-bw-agents.tex <==
\begin{tikzpicture}[node distance=1pt and 16pt]
    \node (n) {\input{img/examples/classical-bw/classical-bw.tex}};

    \node[outer sep=40pt, label={[below, label distance=-50pt, rotate=  0]:\faEye[regular]}] at (n.north)      [above]       {$a$};
    \node[outer sep=6pt,  label={[below, label distance=-18pt, rotate= 30]:\faEye[regular]}] at (n.north west) [above left]  {$l$};
    \node[outer sep=6pt,  label={[below, label distance=-18pt, rotate=-40]:\faEye[regular]}] at (n.north east) [above right] {$r$};
\end{tikzpicture}


==> img/examples/non-det-public-ontic/b1-on-b4.tex <==
\begin{tikzpicture}[node distance=1pt and 16pt]
    \node[wblock] (b0)                   {};
    \node[block]  (b3) [right=of b0]     {$b_3$};
    \node[block]  (b2) [above=of b3]     {$b_2$};
    \node[block]  (b4) [right=of b3]     {$b_4$};
    \node[block]  (b1) [above=of b4]     {$b_1$};

    \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b0.south) -- ([xshift=104pt,yshift=-2pt]b0.south);

    \node[stack] (s1) [below=4pt of b0] {$c_1$};
    \node[stack] (s2) [right=of s1]     {$c_2$};
    \node[stack] (s3) [right=of s2]     {$c_3$};
\end{tikzpicture}

% \begin{tikzpicture}[node distance=1pt and 16pt]
%     \node[block, draw=white] (b0)                   {};
%     \node[block]             (b3) [right=of b0]     {$b_3$};
%     \node[block]             (b2) [above=of b3]     {$b_2$};
%     \node[block]             (b4) [right=of b3]     {$b_4$};

%     \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b0.south) -- ([xshift=104pt,yshift=-2pt]b0.south);

%     \node[stack]             (s1) [below=4pt of b0] {$c_1$};
%     \node[stack]             (s2) [right=of s1]     {$c_2$};
%     \node[stack]             (s3) [right=of s2]     {$c_3$};
% \end{tikzpicture}


==> img/examples/non-det-public-ontic/b4-on-b1.tex <==
\begin{tikzpicture}[node distance=1pt and 16pt]
    \node[block]  (b1)                   {$b_1$};
    \node[block]  (b3) [right=of b1]     {$b_3$};
    \node[block]  (b2) [above=of b3]     {$b_2$};
    \node[block]  (b4) [above=of b1]     {$b_4$};

    \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b1.south) -- ([xshift=104pt,yshift=-2pt]b1.south);

    \node[stack] (s1) [below=4pt of b1] {$c_1$};
    \node[stack] (s2) [right=of s1]     {$c_2$};
    \node[stack] (s3) [right=of s2]     {$c_3$};
\end{tikzpicture}

% \begin{tikzpicture}[node distance=1pt and 16pt]
%     \node[block, draw=white] (b0)                   {};
%     \node[block]             (b3) [right=of b0]     {$b_3$};
%     \node[block]             (b2) [above=of b3]     {$b_2$};
%     \node[block]             (b4) [right=of b3]     {$b_4$};

%     \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b0.south) -- ([xshift=104pt,yshift=-2pt]b0.south);

%     \node[stack]             (s1) [below=4pt of b0] {$c_1$};
%     \node[stack]             (s2) [right=of s1]     {$c_2$};
%     \node[stack]             (s3) [right=of s2]     {$c_3$};
% \end{tikzpicture}


==> img/examples/non-det-public-ontic/ndpo-es.tex <==
\begin{tikzpicture}[node distance=32pt and 64pt, >=stealth']
    \node[graphicaldworld, scale=0.6, label=below:{$w$}] (w) {\input{img/examples/partial-observability/moved-block.tex}};

    \path
        (w) edge[->,  thick, loop, out=105, in= 75, looseness=4] node[above] {$\agentStyle{a},\agentStyle{l},\agentStyle{r}$} (w)
    ;
\end{tikzpicture}


==> img/examples/non-det-public-ontic/ndpo-es_.tex <==
\begin{tikzpicture}[node distance=64pt, >=stealth']
    \node[graphicaldworld,              scale=0.6, label=below:{$(w, e)$}] (we) {\input{img/examples/non-det-public-ontic/b1-on-b4.tex}};
    \node[graphicaldworld, below=of we, scale=0.6, label=below:{$(w, f)$}] (wf) {\input{img/examples/non-det-public-ontic/b4-on-b1.tex}};

    \path
        (we) edge[->,  thick, loop, out=105, in= 75, looseness=4] node[above] {$\agentStyle{a},\agentStyle{l},\agentStyle{r}$} (we)
        (wf) edge[->,  thick, loop, out=105, in= 75, looseness=4] node[above] {$\agentStyle{a},\agentStyle{l},\agentStyle{r}$} (wf)
    ;
\end{tikzpicture}


==> img/examples/non-det-public-ontic/ndpo.tex <==
\begin{tikzpicture}[node distance=48pt, >=stealth', baseline=(e)]
    \node[devent,             label=below:{$e$}] (e) {};
    \node[devent, right=of e, label=below:{$f$}] (f) {};

    \path
        (e) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$\agentStyle{a},\agentStyle{l},\agentStyle{r}$} (e)
        (f) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$\agentStyle{a},\agentStyle{l},\agentStyle{r}$} (f)
    ;
\end{tikzpicture}


==> img/examples/non-determinism/sensing-es.tex <==
\begin{tikzpicture}[node distance=32pt and 32pt, >=stealth']
    \node[graphicaldworld, scale=0.6, label=below:{$u_1$}] (u1)                {\input{img/examples/single-agent-bw/single-agent-bw-1.tex}};
    \node[graphicaldworld, scale=0.6, label=below:{$u_2 $}] (u2) [right=of u1] {\input{img/examples/single-agent-bw/single-agent-bw-2.tex}};

    \path
        (u1) edge[->,  thick, loop, out=105, in= 75, looseness=4] node[above] {$a,l,r$} (u1)
        (u2) edge[->,  thick, loop, out=105, in= 75, looseness=4] node[above] {$a,l,r$} (u2)
    ;
\end{tikzpicture}


==> img/examples/non-determinism/sensing.tex <==
\begin{tikzpicture}[node distance=32pt and 64pt, >=stealth']
    \node[devent, label=below:{$f_1: On(b_2, b_1)~~~~~$}] (f1)               {};
    \node[devent, label=below:{$~~~~~f_2: On(b_2, c_1)$}] (f2) [right=of f1] {};

    \path
        (f1) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$\tau_f$} (f1)
        (f2) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$\tau_f$} (f2)
    ;
\end{tikzpicture}


==> img/examples/partial-observability/fully-oblivious-aem.tex <==
\begin{tikzpicture}[node distance=32pt and 48pt, >=stealth']
    \node[devent, label=below:{$f_1 : \langle pre, post \rangle~~~~~~$}] (f1)               {};
    \node[event,  label=below:{$~~f_2 : \top~~$}]  (f2) [right=of f1] {};

    \path
        (f1) edge[->, thick] node[above] {$\tau_o$} (f2)
        (f1) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$\tau_f$} (f1)
        (f2) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$\tau_f, \tau_o$} (f2)
    ;
\end{tikzpicture}


==> img/examples/partial-observability/fully-oblivious-em-1.tex <==
\begin{tikzpicture}[node distance=32pt and 64pt, >=stealth']
    \node[devent, label=below:{$e_1 : \langle pre, post \rangle~~~$}] (e1)               {};
    \node[event,  label=below:{$e_2 : \top$}]  (e2) [right=of e1] {};

    \path
        (e1) edge[->, thick] node[above] {$a,r$} (e2)
        (e1) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$l$} (e1)
        (e2) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$a,l,r$} (e2)
    ;
\end{tikzpicture}


==> img/examples/partial-observability/fully-oblivious-em-2.tex <==
\begin{tikzpicture}[node distance=32pt and 64pt, >=stealth']
    \node[devent, label=below:{$e'_1 : \langle pre, post \rangle~~~$}] (e1)               {};
    \node[event,  label=below:{$e'_2 : \top$}]  (e2) [right=of e1] {};

    \path
        (e1) edge[->, thick] node[above] {$r$} (e2)
        (e1) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$a,l$} (e1)
        (e2) edge[->, thick, loop, out=130, in=50, looseness=8] node[above] {$a,l,r$} (e2)
    ;
\end{tikzpicture}


==> img/examples/partial-observability/fully-oblivious-es.tex <==
\begin{tikzpicture}[node distance=32pt and 64pt, >=stealth']
    \node[graphicaldworld, scale=0.6, label=below:      {$u_1$}] (u1)                                   {\input{img/examples/partial-observability/moved-block.tex}};
    \node[graphicalworld,  scale=0.6, label=below left: {$u_2$}] (u2) [above left=32pt and -12pt of u1] {\input{img/examples/single-agent-bw/single-agent-bw-1.tex}};
    \node[graphicalworld,  scale=0.6, label=below right:{$u_3$}] (u3) [right=of u2]                     {\input{img/examples/single-agent-bw/single-agent-bw-2.tex}};

    \path
        (u1) edge[->,  thick] node[left]  {$a,r~$} (u2)
        (u1) edge[->,  thick] node[right] {$~a,r$} (u3)
        (u2) edge[<->, thick] node[above] {$a,r$} (u3)
        (u1) edge[->,  thick, loop, out= 10, in=-10, looseness=4] node[right] {$l$}     (u1)
        (u2) edge[->,  thick, loop, out=105, in= 75, looseness=4] node[above] {$a,l,r$} (u2)
        (u3) edge[->,  thick, loop, out=105, in= 75, looseness=4] node[above] {$a,l,r$} (u3)
    ;
\end{tikzpicture}


==> img/examples/partial-observability/moved-block.tex <==
\begin{tikzpicture}[node distance=1pt and 16pt]
    \node[block] (b1)                   {$b_1$};
    \node[block] (b3) [right=of b1]     {$b_3$};
    \node[block] (b2) [above=of b3]     {$b_2$};
    \node[block] (b4) [right=of b3]     {$b_4$};

    \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b1.south) -- ([xshift=104pt,yshift=-2pt]b1.south);

    \node[stack] (s1) [below=4pt of b1] {$c_1$};
    \node[stack] (s2) [right=of s1]     {$c_2$};
    \node[stack] (s3) [right=of s2]     {$c_3$};
\end{tikzpicture}

% \begin{tikzpicture}[node distance=1pt and 16pt]
%     \node[block, draw=white] (b0)                   {};
%     \node[block]             (b3) [right=of b0]     {$b_3$};
%     \node[block]             (b2) [above=of b3]     {$b_2$};
%     \node[block]             (b4) [right=of b3]     {$b_4$};

%     \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b0.south) -- ([xshift=104pt,yshift=-2pt]b0.south);

%     \node[stack]             (s1) [below=4pt of b0] {$c_1$};
%     \node[stack]             (s2) [right=of s1]     {$c_2$};
%     \node[stack]             (s3) [right=of s2]     {$c_3$};
% \end{tikzpicture}


==> img/examples/single-agent-bw/single-agent-bw-1.tex <==
\begin{tikzpicture}[node distance=1pt and 16pt]
    \node[block,dashed] (b1)                   {$\objectStyle{b}_1$};
    \node[block]        (b2) [above=of b1]     {$\objectStyle{b}_2$};
    \node[block]        (b3) [right=of b1]     {$\objectStyle{b}_3$};
    \node[block]        (b4) [right=of b3]     {$\objectStyle{b}_4$};

    \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b1.south) -- ([xshift=104pt,yshift=-2pt]b1.south);

    \node[stack]        (s1) [below=4pt of b1] {$\objectStyle{c}_1$};
    \node[stack]        (s2) [right=of s1]     {$\objectStyle{c}_2$};
    \node[stack]        (s3) [right=of s2]     {$\objectStyle{c}_3$};
\end{tikzpicture}


==> img/examples/single-agent-bw/single-agent-bw-2.tex <==
\begin{tikzpicture}[node distance=1pt and 16pt]
    \node[block]        (b2)                   {$\objectStyle{b}_2$};
    \node[block,dashed] (b1) [right=of b2]     {$\objectStyle{b}_1$};
    \node[block]        (b3) [above=of b1]     {$\objectStyle{b}_3$};
    \node[block]        (b4) [right=of b1]     {$\objectStyle{b}_4$};

    \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b2.south) -- ([xshift=104pt,yshift=-2pt]b2.south);

    \node[stack]        (s1) [below=4pt of b2] {$\objectStyle{c}_1$};
    \node[stack]        (s2) [right=of s1]     {$\objectStyle{c}_2$};
    \node[stack]        (s3) [right=of s2]     {$\objectStyle{c}_3$};
\end{tikzpicture}


==> img/examples/single-agent-bw/single-agent-bw-3.tex <==
\begin{tikzpicture}[node distance=1pt and 16pt]
    \node[block]        (b2)                   {$\objectStyle{b}_2$};
    \node[block]        (b3) [right=of b2]     {$\objectStyle{b}_3$};
    \node[block,dashed] (b1) [right=of b3]     {$\objectStyle{b}_1$};
    \node[block]        (b4) [above=of b1]     {$\objectStyle{b}_4$};

    \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b2.south) -- ([xshift=104pt,yshift=-2pt]b2.south);

    \node[stack]        (s1) [below=4pt of b2] {$\objectStyle{c}_1$};
    \node[stack]        (s2) [right=of s1]     {$\objectStyle{c}_2$};
    \node[stack]        (s3) [right=of s2]     {$\objectStyle{c}_3$};
\end{tikzpicture}


==> img/examples/single-agent-bw/single-agent-bw-after-move.tex <==
\begin{tikzpicture}[node distance=1pt and 16pt]
    \node[block] (b1)                   {$b_1$};
    \node[block] (b3) [right=of b1]     {$b_3$};
    \node[block] (b2) [above=of b3]     {$b_2$};
    \node[block] (b4) [right=of b3]     {$b_4$};

    \draw[gray, very thick] ([xshift=-30pt,yshift=-2pt]b1.south) -- ([xshift=104pt,yshift=-2pt]b1.south);

    \node[stack] (s1) [below=4pt of b1] {$c_1$};
    \node[stack] (s2) [right=of s1]     {$c_2$};
    \node[stack] (s3) [right=of s2]     {$c_3$};
\end{tikzpicture}


==> img/examples/single-agent-bw/single-agent-es-after-action.tex <==
\begin{tikzpicture}[node distance=32pt and 64pt, >=stealth']
    \node[graphicaldworld, scale=0.75, label=below:$w'_1$] (w1) {\input{img/examples/single-agent-bw/single-agent-bw-after-move.tex}};

    \path
        (w1) edge[->,  thick, loop, out=105, in= 75, looseness=4] (w1)
    ;
\end{tikzpicture}

